Hermitian-Lifted Codes

In this paper, we construct codes for local recovery of erasures with high availability and constant-bounded rate from the Hermitian curve. These new codes, called Hermitian-lifted codes, are evaluation codes with evaluation set being the set of $\mathbb{F}_{q^2}$-rational points on the affine curve. The novelty is in terms of the functions to be evaluated; they are a special set of monomials which restrict to low degree polynomials on lines intersected with the Hermitian curve. As a result, the positions corresponding to points on any line through a given point act as a recovery set for the position corresponding to that point.

==> mainthm.tex <==
Our main result is that \ourcodes \ have rate bounded below by a constant independent of $q$.

Note that it is easy to see that $\cC$ has rate at least $\frac{q(q+1)}{2q^3} \geq \frac{1}{2q}$, since $C_{q,q^2-1}$ is a subcode of $\cC$ and the dimension of $C_{q,q^2-1}$ is $\frac{q(q+1)}{2}$. 
%Indeed, 
% $\cC$ contains as a subcode the one-point Hermitian code $\cC_0$ that corresponds to the set of functions $f(x,y)$ of total degree at most $q-1$.  
%(That is, $\cC_0$ is the evaluations of $\mathcal{F}_0 = \inset{ f \in \F_{q^2}[x,y] \suchthat \deg(f) \leq q-1 }$.)
%The dimension of $\cC_0$ is ${ q + 1 \choose 2 }$, and so the dimension of $\cC$ is at least as large.

However, what may be surprising is that in fact there are many functions $f \in \mathcal{F} \setminus \mathcal{F}_0$, enough so that the rate of the code $\cC$ is actually bounded below by a constant independent of $q$.

\begin{theorem}\label{thm:main}
Suppose that $q \geq 4$ is a power of $2$, and let $\cC$ be as in Definition~\ref{def:C}.  Then the rate of $\cC$ is at least $0.007$.  \mkw{I bet we could get a better bound on the rate by being a bit more careful in counting monomials (eg, coming up with more monomials that satisfy thm \ref{lem:tpower}), but it's not going to be high rate no matter what so I'm not sure if it's worth it.}
\end{theorem}




